DiffPack: A Torsional Diffusion Model for Autoregressive Protein Side-Chain Packing

Proteins play a critical role in carrying out biological functions, and their 3D structures are essential in determining their functions. Accurately predicting the conformation of protein side-chains given their backbones is important for applications in protein structure prediction, design and protein-protein interactions. Traditional methods are computationally intensive and have limited accuracy, while existing machine learning methods treat the problem as a regression task and overlook the restrictions imposed by the constant covalent bond lengths and angles. In this work, we present DiffPack, a torsional diffusion model that learns the joint distribution of side-chain torsional angles, the only degrees of freedom in side-chain packing, by diffusing and denoising on the torsional space. To avoid issues arising from simultaneous perturbation of all four torsional angles, we propose autoregressively generating the four torsional angles from $\chi_1$ to $\chi_4$ and training diffusion models for each torsional angle. We evaluate the method on several benchmarks for protein side-chain packing and show that our method achieves improvements of $11.9\%$ and $13.5\%$ in angle accuracy on CASP13 and CASP14, respectively, with a significantly smaller model size ($60\times$ fewer parameters). Additionally, we show the effectiveness of our method in enhancing side-chain predictions in the AlphaFold2 model. Code is available at https://github.com/DeepGraphLearning/DiffPack.

==> section/rebuttal/review_0.tex <==
\newpage
\setcounter{figure}{0}  % TODO
\setcounter{table}{0}  % TODO
\setcounter{section}{0}
\setcounter{page}{1}

\section{Calibration of Confidence Scores}
\vspace{-10pt}

\begin{figure}[H]
    \centering
    \includegraphics[width=0.7\textwidth]{figure/confidence_selection.pdf}
    \caption{\textbf{Percentage of accurate angles as number of samples increasing}. "Oracle Selection" denotes selecting the conformation with lowest RMSD. "Confidence Selection" denotes selecting by trained confidence module.}
\end{figure}
\vspace{-10pt}

% \begin{table}[H]
%     \centering
%     \begin{adjustbox}{max width=0.8\linewidth}
%     \begin{tabular}{lcccc|cccc}
%     \toprule

%             & \multicolumn{4}{c}{Samples=4} & \multicolumn{4}{c}{Samples=1}\\
%                     \cmidrule(lr){ 2 - 9 }  
%          \textbf{Method} & $\chi_1$ & $\chi_2$ & $\chi_3$ & $\chi_4$ & $\chi_1$ & $\chi_2$ & $\chi_3$ & $\chi_4$ \\
%     \midrule
%         \method        & \textbf{15.35} & \textbf{19.19} & \textbf{37.30} & \textbf{50.19} & \textbf{16.12}&	\textbf{22.92}&	\textbf{39.92}&	\textbf{50.63} \\
%     \midrule
%         AttnPacker & 18.79 & 23.21 & 44.63 & 58.72 & 18.92  & 23.17 & 44.89 & 58.98\\
%         DLPacker &-&	-&	-&	- & 22.18 & 27.00 & 51.22 & 70.04\\
%     \bottomrule
%     \end{tabular}
%     \end{adjustbox}
%     \vspace{3pt}
%     \caption{\textbf{Ablation study for multi-sample generation of deep learning models}. DLPacker do not have multiple samples as it's designed without randomness.}
%     \vspace{-15pt}
%     \label{tab:ablation_sample}
% \end{table}
\vspace{-10pt}

\section{Inference Time}
\vspace{-10pt}

\begin{figure}[H]
    \centering
    \includegraphics[width=0.7\textwidth]{figure/speed_comparison.pdf}
    \caption{\textbf{Comparision of speed and accuracy between different methods.} Inference speed is shown in log-scale.}
\end{figure}
\vspace{-10pt}

\begin{table}[H]
    \centering
    \begin{adjustbox}{max width=0.7\linewidth}
    \begin{tabular}{lc|c}
    \toprule
         & \multicolumn{1}{c}{\textsc{Inference Time(s)} $\downarrow$} & \multicolumn{1}{c}{\textsc{Angle Accuracy} $\uparrow$} \\
    \midrule
        SCWRL               & 2.71 &  56.2\% \\ 
        FASPR               & \textbf{0.10} &  56.4\%  \\
        
        RosettaPacker       &  217.80    &  58.6\%   \\
        DLPacker$^\dagger$       &  28.50    &  58.8\%   \\
    AttnPacker$^\dagger$
    &   6.33    &  62.1\%   \\
    \midrule
        DiffPack-vanila$^\dagger$            &  1.29 & \textbf{67.0\%}   \\
        % DiffPack-confidence            &  4.78 & 69.4\%   \\
        % DiffPack-full            &  19.86 & 69.5\%   \\
        DiffPack-dgl$^\dagger$ &  0.69 & \textbf{67.0\%}  \\
    \bottomrule
    \end{tabular}
    \end{adjustbox}
    \vspace{3pt}
    \caption{\textbf{Average Inference Time of Different Methods}.}
    \vspace{-10pt}
\end{table}
\vspace{-10pt}



==> section/rebuttal/reviewer_1.tex <==
\newpage
\setcounter{figure}{0}  % TODO
\setcounter{table}{0}  % TODO
\setcounter{section}{0}
\setcounter{page}{1}

\section{Calibration of Confidence Scores}

\begin{figure}[H]
    \centering
    \includegraphics[width=0.7\textwidth]{figure/confidence_selection.pdf}
    \caption{\textbf{Percentage of accurate angles as number of samples increasing}. "Oraca Selection" denotes selecting the conformation with lowest RMSD. "Confidence Selection" denotes selecting by trained confidence module.}
\end{figure}

\begin{table}[H]
    \centering
    \begin{adjustbox}{max width=0.8\linewidth}
    \begin{tabular}{lcccc|cccc}
    \toprule

            & \multicolumn{4}{c}{Samples=4} & \multicolumn{4}{c}{Samples=1}\\
                    \cmidrule(lr){ 2 - 9 }  
         \textbf{Method} & $\chi_1$ & $\chi_2$ & $\chi_3$ & $\chi_4$ & $\chi_1$ & $\chi_2$ & $\chi_3$ & $\chi_4$ \\
    \midrule
        \method        & \textbf{15.35} & \textbf{19.19} & \textbf{37.30} & \textbf{50.19} & \textbf{16.12}&	\textbf{22.92}&	\textbf{39.92}&	\textbf{50.63} \\
    \midrule
        AttnPacker & 15.31 & 19.17 & 37.18 & 51.02 & 15.35 & 19.19 & 37.30 & 50.19\\
        DLPacker &-&	-&	-&	- & 22.18 & 27.00 & 51.22 & 70.04\\
    \bottomrule
    \end{tabular}
    \end{adjustbox}
    \vspace{3pt}
    \caption{\textbf{Ablation study for multi-sample generation of deep learning models}. DLPacker do not have multiple samples as it's designed without randomness}
    \vspace{-15pt}
    \label{tab:ablation_sample}
\end{table}




==> section/rebuttal/reviewer_2.tex <==
\newpage
\setcounter{figure}{0}  % TODO
\setcounter{table}{0}  % TODO
\setcounter{section}{0}
\setcounter{page}{1}

\section{Inference Time}
\vspace{-10pt}

\begin{figure}[H]
    \centering
    \includegraphics[width=0.7\textwidth]{figure/speed_comparison.pdf}
    \caption{\textbf{Comparision of speed and accuracy between different methods.} Inference speed is shown in log-scale}
\end{figure}

\begin{table}[H]
    \centering
    \begin{adjustbox}{max width=0.7\linewidth}
    \begin{tabular}{lc|c}
    \toprule
         & \multicolumn{1}{c}{\textsc{Inference Time(s)} $\downarrow$} & \multicolumn{1}{c}{\textsc{Angle Accuracy} $\uparrow$} \\
    \midrule
        SCWRL               & 2.71 &  56.2\% \\ 
        FASPR               & \textbf{0.10} &  56.4\%  \\
        
        RosettaPacker       &  217.80    &  58.6\%   \\
        DLPacker$^\dagger$       &  28.50    &  58.8\%   \\
    AttnPacker$^\dagger$
    &   6.33    &  62.1\%   \\
    \midrule
        DiffPack-vanila$^\dagger$            &  1.29 & \textbf{67.0\%}   \\
        % DiffPack-confidence            &  4.78 & 69.4\%   \\
        % DiffPack-full            &  19.86 & 69.5\%   \\
    \bottomrule
    \end{tabular}
    \end{adjustbox}
    \vspace{3pt}
    \caption{\textbf{Average Inference Time of Different Methods}}
    \vspace{-10pt}
\end{table}

\section{Confidence Selection}
\begin{figure}[H]
    \centering
    \includegraphics[width=0.7\textwidth]{figure/confidence_selection.pdf}
    \caption{\textbf{Percentage of accurate angles as number of samples increasing}. "Oraca Selection" denotes selecting the conformation with lowest RMSD. "Confidence Selection" denotes selecting by trained confidence module.}
\end{figure}


==> section/rebuttal/reviewer_3.tex <==
\newpage
\setcounter{figure}{0}  % TODO
\setcounter{table}{0}  % TODO
\setcounter{section}{0}
\setcounter{page}{1}

\section{Inference Time}
\vspace{-10pt}

\begin{figure}[H]
    \centering
    \includegraphics[width=0.7\textwidth]{figure/speed_comparison.pdf}
    \caption{\textbf{Comparision of speed and accuracy between different methods.} Inference speed is shown in log-scale}
\end{figure}

\begin{table}[H]
    \centering
    \begin{adjustbox}{max width=0.7\linewidth}
    \begin{tabular}{lc|c}
    \toprule
         & \multicolumn{1}{c}{\textsc{Inference Time(s)} $\downarrow$} & \multicolumn{1}{c}{\textsc{Angle Accuracy} $\uparrow$} \\
    \midrule
        SCWRL               & 2.71 &  56.2\% \\ 
        FASPR               & \textbf{0.10} &  56.4\%  \\
        
        RosettaPacker       &  217.80    &  58.6\%   \\
        DLPacker$^\dagger$       &  28.50    &  58.8\%   \\
    AttnPacker$^\dagger$
    &   6.33    &  62.1\%   \\
    \midrule
        DiffPack-vanila$^\dagger$            &  1.29 & \textbf{67.0\%}   \\
        % DiffPack-confidence            &  4.78 & 69.4\%   \\
        % DiffPack-full            &  19.86 & 69.5\%   \\
    \bottomrule
    \end{tabular}
    \end{adjustbox}
    \vspace{3pt}
    \caption{\textbf{Average Inference Time of Different Methods}}
    \vspace{-10pt}
\end{table}


==> section/rebuttal/reviewer_4.tex <==
\newpage
\setcounter{figure}{0}  % TODO
\setcounter{table}{0}  % TODO
\setcounter{section}{0}
\setcounter{page}{1}

\section{Inference Time}
\vspace{-10pt}

\begin{figure}[H]
    \centering
    \includegraphics[width=0.7\textwidth]{figure/speed_comparison.pdf}
    \caption{\textbf{Comparision of speed and accuracy between different methods.} Inference speed is shown in log-scale}
\end{figure}

\begin{table}[H]
    \centering
    \begin{adjustbox}{max width=0.7\linewidth}
    \begin{tabular}{lc|c}
    \toprule
         & \multicolumn{1}{c}{\textsc{Inference Time(s)} $\downarrow$} & \multicolumn{1}{c}{\textsc{Angle Accuracy} $\uparrow$} \\
    \midrule
        SCWRL               & 2.71 &  56.2\% \\ 
        FASPR               & \textbf{0.10} &  56.4\%  \\
        
        RosettaPacker       &  217.80    &  58.6\%   \\
        DLPacker$^\dagger$       &  28.50    &  58.8\%   \\
    AttnPacker$^\dagger$
    &   6.33    &  62.1\%   \\
    \midrule
        DiffPack-vanila$^\dagger$            &  1.29 & \textbf{67.0\%}   \\
        % DiffPack-confidence            &  4.78 & 69.4\%   \\
        % DiffPack-full            &  19.86 & 69.5\%   \\
    \bottomrule
    \end{tabular}
    \end{adjustbox}
    \vspace{3pt}
    \caption{\textbf{Average Inference Time of Different Methods}}
    \vspace{-10pt}
\end{table}

